Incorporating Human Path Preferences in Robot Navigation with Minimal Interventions

Robots that can effectively understand human intentions from actions are crucial for successful human-robot collaboration. In this work, we address the challenge of a robot navigating towards an unknown goal while also accounting for a human's preference for a particular path in the presence of obstacles. This problem is particularly challenging when both the goal and path preference are unknown a priori. To overcome this challenge, we propose a method for encoding and inferring path preference online using a partitioning of the space into polytopes. Our approach enables joint inference over the goal and path preference using a stochastic observation model for the human. We evaluate our method on an unknown-goal navigation problem with sparse human interventions, and find that it outperforms baseline approaches as the human's inputs become increasingly sparse. We find that the time required to update the robot's belief does not increase with the complexity of the environment, which makes our method suitable for online applications.

==> _previous_versions/2023_02_13/1_Introduction.tex <==
Consider a robot carrying a table through an office. The robot must navigate around people and obstacles towards a pre-specified target location. However, its sensing and planning capabilities may not be able to detect the spilt coffee in the hall, nor predict that one of the workers is leaving their desk and needs a clear passage to reach their bag on the opposite side. On the other hand, a human has the ability to understand the context of a mission and quickly adjust by finding alternative ways to execute the task.

When deploying robots around humans in the real world, adjusting to such unexpected situations in a timely manner is crucial for ensuring human safety. When a robot cannot perceive a danger or lacks situational awareness, the human can provide recommendations to the robot, either in the form of actions (the human is also pushing the table) or remote instructions (joystick or other form of teleoperation). However, in today's shared autonomy frameworks for human-robot collaboration, the fully autonomous robot is not likely to comply with the human's recommendation if it conflicts with the goal of the task.
An alternative option is to make the robot more compliant, which requires the human to intervene more frequently, thus wasting time and energy by providing the robot with redundant information. Furthermore, when the robot needs to infer the goal of a task from human observations, such unexpected deviations deteriorate the quality of predictions and make the task less likely to be correctly executed.

We claim that such behaviors in human-robot autonomy are due to the assumption that the \emph{goal} of a task (e.g. target location) and the human's \emph{preference} on how to execute the task (e.g. which path to take) are tightly coupled. 

Our contribution are as follows.
\begin{itemize}
    \item We formulate the human-robot collaborative object transport problem as a Partially Observable Markov Decision Process (POMDP) where both the goal of the task and the human's path preference are unknown random variables.
    \item We build a framework for solving the aforementioned POMDP online over a two-dimensional office map
    \item We conduct a real-world case study where a human collaborates with a fleet of autonomous omnidirectional robot platforms (Ouijabots) to transport an object through an office, and show that our solution [requires that much less control effort] compared with a compliant baseline, and [takes that much less time to complete the task] compared to a solution that ignores path preference.
\end{itemize}


% How it works (bayesian intention inference)
% - Representation is sparse
% - We pull out a graphical model from what we think the human preference pattern is (accounting only for obstacles in the local region)
% - method is tractable

% - Method works in sim and hardware
% - We minimize the human intervention effort AND task execution time compared to inferring goal only or path only.





% are not always sufficient to determing the best path to the goal. For example, the robot may not predict that one of the workers will want to 
% When deploying such a system in the real world, not ac

% A human's time is a precious resource
% Human intervention must be sparse and effective.

% In shared autonomy problems, while a lot of emphasis has been placed on inferring a goal, objective or cost functions of a human as inherently associated with to a specific task, accounting for human preference on \emph{how} to execute an instance of a task has not received as much attention.

% If the conditions are \emph{perfect}, the robot has sufficient knowledge of the environment to carry out the task autonomously.
% However, the robot's sensors and mapping capabilities are not enough to ac

% Unfortunately, when operating in dynamic environments and in spaces with other humans involved, 

% In many applications where human and robotic agents interact, the ability to predict a human’s intention is key. In autonomous driving, predicting a distribution of possible pedestrian trajectories from human intention is important to make safe navigation decisions. In collaborative object transport tasks, human intention may include a goal destination and a preferred path towards this goal that a robot should help to assist towards.

% In the recent literature for intent inference applied to such problems, human path preferences (turning right/left etc) are not encoded in the belief space. This poses a problem as the human’s preferred path towards a goal does not always match the path that the robot would optimize for for this same goal, especially when the environment is cluttered or complex.

% Contribution: We show that by leveraging generative models that account for human homotopic preferences, we can enrich / better inform our belief and improve both shared autonomy and trajectory prediction algorithms.


% There could be various reasons for a human to make a homotopic choice.
% - obstacles in the way or any difficulty that the robot does not see
% - It is simpler for the human to navigate there (wider passage, or human motion is simpler, less effort that the robot didn't account for)
% - information provided by another human about something that will happen in the future at this location
% - things that may happen at this location
% - failure of the robot to detect this path??
% - an instruction that the robot does not have access to
% - other path just looks better

% We could use heuristics to account for these features (and we should try it out), but it will be difficult to account for everything in a realistic way and that works for all humans in different environments (without overfitting). To account for these things that our software is not able to predict, we need to accept that the human can make a homotopic choice with some probability.


==> _previous_versions/2023_02_13/3_Problem_Statement.tex <==
\input{tickx_graphics/BII_diagram_policy_combined.tex}


We consider a single robot navigating in an environment.
Let $S_t$ be the physical location of the robot at time index $t$. The transition model $T(s_{t+1} \mid s_t,a_t)$ is deterministic, i.e. the robot has full control over its future location. At any time step, the human may provide observations for the robot. The observation $o_t$ corresponds to either a joystick input or forces that are applied by a human on the robot. In practice, an observation can be either a wrench applied by the human on the object, or a joystick command. In this work, we assume that the observation the robot makes of the human actions is a direction.

The robot is given a stochastic observation model for the human $\mathcal{O}(o_t \mid s_t, g, \pi)$ conditioned both on the goal of the task $g$, and the human's preferred policy $\pi$, which we introduce in this paper. The diagram is shown in Figure \ref{fig:BII_policy_only}.


\subsection{Human observation model without path preference}

%The human actions are modeled according to a stochastic observation model $o_{t} = f(g) + \epsilon$. 
Observation $o_t$ designates a direction. Taking one step in this direction brings the robot and object to a location $l_t$ in space.

[BII paper] propose the following human model:
\begin{equation}
    P(l_{t} \mid S_t, g)  \; \propto \; e^{-\gamma \big( (\delta(S_t \rightarrow g \mid l_t) - (\delta(S_t \rightarrow g) \big)}
\end{equation}
where $\delta(a,b \mid c)$ is the length of the shortest path in between $a$ and $b$ passing by $c$.

\subsection{Human observation model with path preference}

The previous human observation model is defined conditioned on the goal of the task, but not on \emph{how} to execute the task. In this work, we propose the following human model conditioned on both the goal of the task and the human's preference policy.

1. Human policy: $\pi(S_{t})$ designates the human's preferred path from state $S_t$. We call human \emph{intent} at state $S_t$ the joint $\lbrace \pi(S_t),g \rbrace$.

2. $o_{t} = f(\pi(S_{t}), g) + \epsilon$ designates a next location $l_t$

And we propose the human model
\begin{equation}
    \label{eq:humanmodel}
    P(l_{t} \mid S_t, g, \theta)  \; \propto \; e^{-\gamma \big( (\delta(S_t \rightarrow g \mid l_t, \theta) - (\delta(S_t \rightarrow g \mid \theta) \big)}
\end{equation}
where $\pi(S_t)$ designates the human preference, and $\delta(a,b \mid \pi(s))$ designates the shortest path from a to b conditioned on the human path $\pi(s)$.

Note that the path preference $\pi$ does not have to be a sequence of locations - it can designate a homotopy, a sequence of areas to visit...

\subsection{Inference}

At each time step where the human provides an observation, the posterior on the joint $(g,\pi)$ is given through the bayesian update
\begin{equation}
\label{eq:inference}
    P(g,\theta \mid l_{1:t}, S_{1:t})  \; \propto \; P(l_{t} \mid S_t, g, \theta) \times P(g,\theta \mid l_{1:t-1}, S_{1:t-1}).
\end{equation}

\begin{equation}
\label{eq:inference}
    P(g \mid l_{1:t}, S_{1:t})  \; \propto \; P(l_{t} \mid S_t, g) \times P(g \mid l_{1:t-1}, S_{1:t-1}).
\end{equation}

We note that in a discrete policy space, the number of bayesian updates that needed to be conducted at each iteration to update the belief is equal to the cardinality of the joint $(g,\pi)$. We also note that each bayesian update requires solving a constrained shortest path problem from Eq. \ref{eq:humanmodel}. If policy $\pi$ represents a discrete distribution over all possible paths to the goal starting from any current state, the above update is intractable. In the next section, we propose a specific encoding of preference policy $\pi$ for resolving Eq. \ref{eq:inference}.


\subsection{Decision Making}

Finally, the robot leverages its belief on the human intent in order to accomplish the object transportation task.

Define: 
Reward structure, Transition model here. 


% Reasoning over all policies $\pi(s)$ is generally intractable. In the next section, we propose an encoding for $\pi$ for object transport problems so as to make it tractable.





% \input{tickx_graphics/BII_diagram_goal_full.tex}

% \input{tickx_graphics/BII_diagram_policy_full.tex}


% \subsection{Intention Inference with Path Preference}

% Bayesian update over b(g,pi)

% Intractable!



==> _previous_versions/2023_02_13/BII_diagram_policy_full.tex <==

\begin{figure}
\label{fig:BII_diagram_policy_obs}
\begin{tikzpicture}[->,>=stealth',auto,node distance=2.5cm,
  thick]
  
  \tikzstyle{dots} = [circle,text centered]
  \tikzstyle{state} = [circle,draw,fill=black!5, minimum size=1.2cm]
  \tikzstyle{observation} = [circle,draw,fill=blue!5, minimum size=1.2cm]
  \tikzstyle{belief} = [circle,draw,fill=orange!5, minimum size=1.2cm]

  \node[dots] (1) {\dots};
  \node[state] (2) [right of=1] {$S_{t-1}$};
  \node[state] (3) [right of=2] {$S_t$};
  \node[state] (4) [right of=3] {$S_{t+1}$};
  \node[dots] (5) [right of=4] {\dots};
  
  \node[observation] (6) [below of=2] {$o_{t-1}$};
  \node[observation] (7) [below of=3] {$o_t$};
  \node[observation] (8) [below of=4] {$o_{t+1}$};
  
%   \node[belief] (goal) [above of=3] {$g$};
  \node[belief] (goal) [below of=7] {$g, \pi$};

  \path[every node/.style={font=\sffamily\small}]
    (1) edge node [right] {} (2)
    (2) edge node [right] {} (3)
    (3) edge node [right] {} (4)
    (4) edge node [right] {} (5)
    (2) edge node [below] {} (6)
    (3) edge node [below] {} (7)
    (4) edge node [below] {} (8)
    % (goal) edge node [left] {} (3)
    % (goal) edge node [right] {} (4)
    % (goal) edge node [left] {} (2);
    (goal) edge node [left] {} (6)
    (goal) edge node [right] {} (7)
    (goal) edge node [left] {} (8);
    %(4) edge[bend right] node [left] {} (1);
    % (goal) edge [bend right] node [left] (3)
    
    
    \draw [dotted, draw=gray, ->] (goal) -- (2);
    \draw [dotted, draw=gray, ->] (goal) to [bend right] (3);
    \draw [dotted, draw=gray, ->] (goal) -- (4);

\end{tikzpicture}
\caption{Intent inference model for trajectory prediction with path preferences. The belief in the human's planning policy is modeled as a discrete probability distribution over the set of all possible sequences for the solution for each robot location. %For figure simplicity, we removed the dotted lines representing the feed-forward effect of the human actions on the object.
}
\end{figure}


% \begin{figure}
% \label{BII_diagram_complete}
% \begin{tikzpicture}[->,>=stealth',auto,node distance=2.5cm,
%   thick]
  
%   \tikzstyle{dots} = [circle,text centered]
%   \tikzstyle{state} = [circle,draw,fill=black!5, minimum size=1.2cm]
%   \tikzstyle{belief} = [circle,draw,fill=orange!5, minimum size=1.2cm]

%   \node[dots] (1) {\dots};
%   \node[state] (2) [right of=1] {$S_{t-1}$};
%   \node[state] (3) [right of=2] {$S_t$};
%   \node[state] (4) [right of=3] {$S_{t+1}$};
%   \node[dots] (5) [right of=4] {\dots};
  
%   \node[belief] (goal) [above of=3] {$g$, $\pi$};

%   \path[every node/.style={font=\sffamily\small}]
%     (1) edge node [right] {} (2)
%     (2) edge node [right] {} (3)
%     (3) edge node [right] {} (4)
%     (4) edge node [right] {} (5)
%     (goal) edge node [left] {} (3)
%     (goal) edge node [right] {} (4)
%     (goal) edge node [left] {} (2);
%     %(4) edge[bend right] node [left] {} (1);
% \end{tikzpicture}
% \caption{Intent inference model for trajectory prediction with a path preference. 
% % Version 1: The belief in the human's preferred sequence of hyperplanes is modeled as a discrete probability distribution over the set of all possible sequences for the solution. 
% % Version 2: 
% The belief in the human's planning policy is modeled as a discrete probability distribution over the set of all possible sequences for the solution for each robot location.}
% \end{figure}

==> _previous_versions/2023_02_24/1_Introduction.tex <==


% Humans can be effective assistants to robots (robot executes the bulk of the task, and the human provides corrections or recommendations on how to do the task). Consider a robot carrying an object in an environment interacting with humans. If it were alone, the robot could carry out the task on its own. However, because there are people, it needs to be able to work with them, i.e. account for their preferences on how it should do its task.
% 

When humans and robots collaborate and interact with each other, we expect robots to be able to quickly adapt to human decisions. Consider a ground robot navigating inside a busy room to deliver a box. It picks a path to its destination (perhaps the shortest) passing in between occupied desks. The people working at these desks may not appreciate the robot passing and interrupting their discussion. They may also want the robot to make a detour on the right so that their co-worker notices the box being delivered.
These new problem requirements coming from human insight and preferences have the particularity that they cannot be inferred by the robot unless people take specific actions, such as applying a force on the robot or giving a joystick instruction, to indicate the information.

We look at the problem where the robot, an imperfect, partial observer of the environment, makes navigation decisions that a human seeks to influence through recommendations. The more quickly the robot can infer the human's preference from their actions and adapt, the less effort is required from the human to do so. %(Saving the operator's time is critical...)
Solutions to this problem have been explored in the area of shared autonomy, where the robot can either \emph{infer} the human's intention given inputs, \cite{bajcsy2017learning, javdani2015shared}, correct its trajectory online \cite{hagenow2021corrective}, or leave control of a latent action space to a human operator \cite{losey2020controlling, jeon2020shared}. 


\citet{bajcsy2017learning} consider an online adaptation problem in the context of a manipulation task where a person can apply forces on the robot to indicate their preferences. For example, if the robot carries a cup of coffee too far above the ground, they will press the arm downwards and expect the robot to keep the cup at a low height even as they release it, preserving their preference while executing the task. \citet{bajcsy2017learning} frame the problem as a Partially Observable Markov Decision Process (POMDP) where parameters of the reward function are unknown a-priori and can be inferred online from human actions. %The robot's reward is a linear combination of features (e.g. tilt of the cup, or its distance to a human) with their unknown, continuous-valued weights (parameters).
We adopt a similar approach for adaptation to a human's preference in the context where a robot must autonomously navigate in a known environment, such as a cluttered office space. We focus on the particular problem where the human seeks to change the robot's \emph{path} with respect to obstacles, (e.g. contour the desks on the right). 

A common way to represent different categories of paths is using the concept of homotopy classes \cite{bhattacharya2012topological}. %However, the way in we encode path preferences and model human actions conditioned on their preference can pose computational challenges. 
However, using homotopies to encode and infer human preferences can pose computational challenges.
If the robot maintains a belief over homotopy classes for paths in between its current location and the goal, the complexity of the inference problem can grow exponentially with the number of obstacles in the space, making the resulting decision-making problem intractable. Furthermore, when the goal is also a problem unknown (which is commonly seen in prediction and shared autonomy problems such as \cite{best2015bayesian, javdani2015shared}), the number of unknown variables increases linearly with the number of candidate destinations.

% \citet{best2015bayesian} propose an interesting approach for predicting an agent's intended trajectory from observations. Rather than maintaining a belief over the agent's future path, they infer the agent's intended \emph{goal} among a set of candidate locations at the boundary of the space. This encoding of the agent's destination provides information on where it is heading, and this intention distribution is then used to generate a distribution of candidate future trajectories for the agent.

% Inferring the goal of the task among a discrete set of candidates is also relevant to the area of shared autonomy. In shared autonomy, both a person and a robot are active decision-makers and must collaborate to execute a common task. \citet{javdani2015shared} propose a problem formalism for shared control of a robotic arm, where the robot must assist the human in picking up an object but needs to infer \emph{which} object the human has chosen from joystick inputs. As the user guides the arm towards its intended object, the robot updates its belief over the candidate objects until it is confident enough to actively assist the human in picking it up.

% We argue that inferring the goal of the task and inferring a human's preferred homotopic path to a goal should be considered as separate problems. Consider the above shared autonomy scenario where the user wishes to use the robotic arm to pick up an object on the left, but prefers to get around an obstacle on the right. While providing inputs to move around the obstacle, the robot updates its belief and infers that the intended object is most likely on the right. We now face the problem where the robot is \emph{over-confident} in the wrong goal, and the robotic assistance will be more likely to pick up the wrong object. The inherent issue with this model when obstacles are present is that conditioned on a certain goal, the human's behavior is modeled as noisily rational, i.e. the human will pick the lowest cost action (perhaps the shortest path) with the highest probability and the likelihood of its action decreases exponentially with the increase in cost. In our work, we consider instead that left and right side of the obstacle are different modes among(?) which the human can have a preference. (rephrase) The robot infers the path preference jointly with the goal of the task, and we assume the human's behavior is noisily rational conditioned on both the \emph{goal} and the \emph{preference}.

%different modes and that the human may prefer one over the other. (rephrase)
% We argue that carrying out inference over the goal of the task as a proxy for path inference is too strongly limited, because the set of goals and the set of paths cannot be mapped one-to-one.

% The problem of inferring an agent's intended path has been approached in the literature under the hood of goal inference. \cite{best2015bayesian}
% BII and goal inference for shared autonomy

% Furthermore, we target shared autonomy applications (where the human and robot are both active decision makers in a collaborative task, e.g. [hindsight]) where the robot should infer the path preference jointly with the goal of the task and any other unknown parameter of the problem.


This paper addresses how to encode and model a human's path preference such that a robot can update its belief over the path and goal jointly and replan online. The key to our solution is to leverage the fact that the human's actions do not contain information about the entire path at once. For example, we would push the robot on its right to indicate a preference for going around the desk in front of the robot, but this will not contain much information about how to navigate around the tables further ahead. Based on this insight, we encode a preference policy as a set of preferred transitions in between polytopes partitioning the environment and introduce conditional independence assumptions into our model that make the Bayesian inference problem tractable.% (the complexity does not increase exponentially with the number of obstacles).

Our contribution are as follows.
\begin{itemize}
    \item We formulate the human-robot collaboration problem as a Partially Observable Markov Decision Process (POMDP) where both the goal of the task and the human's path preference are unknown random variables.
    \item We propose an encoding of a human's path preference, along with conditional independence assumptions over the problem variables for inferring task goal and path preference online.
    \item (simulation results here) %(without path inference, the robot is over-confident in incorrect goal, resulting in a lower success rate compared to our solution...)
\end{itemize}


% Our contribution are as follows.
% \begin{itemize}
%     \item We formulate the human-robot collaborative object transport problem as a Partially Observable Markov Decision Process (POMDP) where both the goal of the task and the human's path preference are unknown random variables.
%     \item We build a framework for solving the aforementioned POMDP online over a two-dimensional office map
%     \item We conduct a real-world case study where a human collaborates with a fleet of autonomous omnidirectional robot platforms (Ouijabots) to transport an object through an office, and show that our solution [requires that much less control effort] compared with a compliant baseline, and [takes that much less time to complete the task] compared to a solution that ignores path preference.
% \end{itemize}


% In particular, the problem the robot is tasked to solve needs to remain tractable so that it can compute solutions online.





% Consider a robot carrying a table through an office. The robot must navigate around people and obstacles towards a pre-specified target location. However, its sensing and planning capabilities may not be able to detect the spilt coffee in the hall, nor predict that one of the workers is leaving their desk and needs a clear passage to reach their bag on the opposite side. On the other hand, a human has the ability to understand the context of a mission and quickly adjust by finding alternative ways to execute the task.

% When deploying robots around humans in the real world, adjusting to such unexpected situations in a timely manner is crucial for ensuring human safety. When a robot cannot perceive a danger or lacks situational awareness, the human can provide recommendations to the robot, either in the form of actions (the human is also pushing the table) or remote instructions (joystick or other form of teleoperation). However, in today's shared autonomy frameworks for human-robot collaboration, the fully autonomous robot is not likely to comply with the human's recommendation if it conflicts with the goal of the task.
% An alternative option is to make the robot more compliant, which requires the human to intervene more frequently, thus wasting time and energy by providing the robot with redundant information. Furthermore, when the robot needs to infer the goal of a task from human observations, such unexpected deviations deteriorate the quality of predictions and make the task less likely to be correctly executed.

% We claim that such behaviors in human-robot autonomy are due to the assumption that the \emph{goal} of a task (e.g. target location) and the human's \emph{preference} on how to execute the task (e.g. which path to take) are tightly coupled. 




% How it works (bayesian intention inference)
% - Representation is sparse
% - We pull out a graphical model from what we think the human preference pattern is (accounting only for obstacles in the local region)
% - method is tractable

% - Method works in sim and hardware
% - We minimize the human intervention effort AND task execution time compared to inferring goal only or path only.



% are not always sufficient to determing the best path to the goal. For example, the robot may not predict that one of the workers will want to 
% When deploying such a system in the real world, not ac

% A human's time is a precious resource
% Human intervention must be sparse and effective.

% In shared autonomy problems, while a lot of emphasis has been placed on inferring a goal, objective or cost functions of a human as inherently associated with to a specific task, accounting for human preference on \emph{how} to execute an instance of a task has not received as much attention.


% In the recent literature for intent inference applied to such problems, human path preferences (turning right/left etc) are not encoded in the belief space. This poses a problem as the human’s preferred path towards a goal does not always match the path that the robot would optimize for for this same goal, especially when the environment is cluttered or complex.

% Contribution: We show that by leveraging generative models that account for human homotopic preferences, we can enrich / better inform our belief and improve both shared autonomy and trajectory prediction algorithms.


% There could be various reasons for a human to make a homotopic choice.
% - obstacles in the way or any difficulty that the robot does not see
% - It is simpler for the human to navigate there (wider passage, or human motion is simpler, less effort that the robot didn't account for)
% - information provided by another human about something that will happen in the future at this location
% - things that may happen at this location
% - failure of the robot to detect this path??
% - an instruction that the robot does not have access to
% - other path just looks better



==> _previous_versions/2023_02_24/2_Related_Work.tex <==

\citet{best2015bayesian} propose an interesting approach for predicting an agent's intended trajectory from observations. Rather than maintaining a belief over the agent's future path, they infer the agent's intended \emph{goal} among a set of candidate locations at the boundary of the space. This encoding of the agent's destination provides information on where it is heading, and this intention distribution is then used to generate a distribution of candidate future trajectories for the agent.

Inferring the goal of the task among a discrete set of candidates is also relevant to the area of shared autonomy. In shared autonomy, both a person and a robot are active decision-makers and must collaborate to execute a common task. \citet{javdani2015shared} propose a problem formalism for shared control of a robotic arm, where the robot must assist the human in picking up an object but needs to infer \emph{which} object the human has chosen from joystick inputs. As the user guides the arm towards its intended object, the robot updates its belief over the candidate objects until it is confident enough to actively assist the human in picking it up.

We argue that inferring the goal of the task and inferring a human's preferred path to a goal should be considered as separate problems. Consider the above shared autonomy scenario where the user wishes to use the robotic arm to pick up an object on the left, but prefers to get around an obstacle on the right. While providing inputs to move around the obstacle, the robot updates its belief and infers that the intended object is most likely on the right. We now face the problem where the robot is \emph{over-confident} in the wrong goal, and the robotic assistance will be more likely to pick up the wrong object.
In an environment containing obstacles, assuming that the human's behavior is noisily rational conditioned only on the goal will lead to such over-confiden behaviors.
%By noisily rational, the human will pick the lowest cost action (perhaps the shortest path) with the highest probability and the likelihood an action decreases exponentially with the increase in cost. 
In our work, we consider instead that left and right side of the obstacle are modes corresponding to different homotopy classes, one of which is preferred by the human. The robot infers the path preference jointly with the goal of the task, and we assume the human's behavior is noisily rational conditioned on both the goal and the preference.

% A homotopy class of trajectories is defined by the set of
% trajectories joining same start and end points which can be
% smoothly deformed into one another without intersecting obstacles. Multiple homotopy classes arise due to presence of
% obstacles in the environment. Homotopy class constraints
% consist of restricting the solution to certain allowed homotopy classes or forbidding others
Two trajectories belong to the same homotopy class if one can be deformed smoothly into the other without intersecting an obstacle \cite{bhattacharya2012topological}. Planning with homotopy class constraints is useful in problems where the robot's requirements are given with respect to obstacles. For example, \cite{yi2016homotopy} consider topological constraints provided by human operators of the form “go quickly from A to B while avoiding C”. \citet{Bhattacharya_2010} proposed an efficient algorithm for solving path planning problems under homotopic constraints that can apply to such problems.
% Unfortunately, carrying out inference over homotopy classes in a dynamic environment is particularly challenging. 
Unfortunately, the number of homotopy classes for a given problem can be infinite, which makes it challenging to carry out inference over homotopy classes. In addition, homotopies are defined for a given set of obstacles and for a specific start and goal locations. As the robot changes location and updates its representation of the world, carrying out inference over homotopy classes in a dynamic environment requires re-computing the set of homotopies at every iteration, making the belief update challenging.

Our solution is to propose an encoding for path preference based on a partitioning of the obstacle-free space into polytopes \cite{vincent2021reachable}, with the particularity that paths belonging to different homotopy classes correspond to different preferences.


% homotopies from start to goal. Downsides:
% - shortest path homotopies are not always the most relevant
% - homotopy is defined with respect to a start and a goal, and these need to be re-defined as the robot moves, which is especially challenging. In addition, as the number of candidate goals increases, the number of homotopies increase linearly as well (one set of them per goal)
% - Each obstacle adds a new dimension to the problem (for astar with homotopy work), making the complexity increase exponentially with the number of obstacles.

% We propose an encoding for path preference that is similar to the concept of homotopies and defined according to a partitioning of the obstacle-free environment into polytopes. Explain Joe Vincent's work briefly here and more in problem formulation section.

==> _previous_versions/2023_02_24/3_Problem_Statement.tex <==

% NOTATIONS
\newcommand{\location}{S} %
\newcommand{\goal}{g} %
\newcommand{\goalset}{\mathcal{C}(\goal)}
\newcommand{\preference}{\theta}
\newcommand{\preferenceset}{\Theta}
\newcommand{\action}{a}
\newcommand{\observation}{o}
\newcommand{\projectedlocation}{l}


\input{tickx_graphics/BII_diagram_policy_full.tex}

We consider a robot that is tasked to navigate in a known environment to an unknown destination. A human knows the destination and can intervene with a joystick to provide a heading direction to the robot. The human also has a preference on which \emph{path}, with respect to obstacles, the robot should take to get to the goal. Our objective is for the robot to understand the human's intentions and execute the task accordingly while requiring a minimal amount of interventions.

% A person wants to influence \emph{how} the robot is performing the task and gives heading directions to the robot with a joystick. The goal of the task and the human's path preference are both unknown to the robot. Our objective is for the robot to understand the human's preference and execute the task accordingly. % with a minimal amount of control inputs from the human.

Let $\goal$ be a random variable designating the goal of the task. $\goal$ belongs to a discrete set of candidates $\goalset$.
Let $\preference$ be the human's path preference. %We denote $\preferenceset$ the set of possible preferences.
Let $\location_t$ be the physical location of the robot and $\action_t$ the robot's action at time index $t$. The transition model $T(\location_{t+1} \mid \location_t,\action_t)$ is deterministic: the robot has full control over its future location. At any time step, the human may provide observations for the robot. When a human intervenes (either with a joystick or by applying forces on the robot), the robot receives an observation $\observation_t$ corresponding to a direction (i.e. heading angle). Taking one step in direction $\observation_t$ from location $\location_t$ brings the robot and object to a new location $\projectedlocation_t$ in space.

The robot is given a stochastic observation model for the human $\mathcal{O}(\observation_t \mid \location_t, \goal, \preference)$ conditioned both on the goal of the task $\goal$, and the human's preferred path $\preference$, which we introduce in this paper. The diagram is shown in Figure \ref{fig:BII_diagram_policy_obs}.


% -------------------------------------------
%Figure placement
\begin{figure*}
\subfloat[width=6cm][Hyperplane arrangement of a two-dimensional space. The robot is located inside the polytope colored in pink, surrounded by three adjacent obstacle-free polytopes. Each hyperplane on the boundary of the robot's polytope corresponds to one of the non-redundant constraints in Eq. \ref{eq:polytope_h_representation_essential}.]{\resizebox{0.65\columnwidth}{!}{%
\includegraphics[]{figures/hyperplane_arrangement.PNG}}\label{fig:HA}} 
\quad
\subfloat[width=6cm][Graph derived from hyperplane arrangement. The nodes on the graph designate polytopes, and edges designate transitions in between adjacent regions. The robot is assigned to the blue node in the graph, and the human provides inputs according to the goal of the task and their preference over transitions $p_1$, $p_2$ and $p_3$. \blue{notations for p are inconsistent with the rest: need to change the figures}]{\resizebox{0.65\columnwidth}{!}{%
\includegraphics[]{figures/HA_graph.PNG}}\label{fig:HA_graph}}
\quad
\subfloat[width=6cm][Example preference defined over the graph. The location of the goal is indicated with the yellow pentagon in the lower right polytope. For each node, the outgoing pink arrow designates the edge on the graph corresponding to the preferred transition in between polytopes.]{\resizebox{0.65\columnwidth}{!}{%
\includegraphics[]{figures/HA_pref.PNG}}\label{fig:HA_pref}}
\caption{Using the hyperplanes composing the H-representation of each obstacle, we construct a hyperplane arrangement of the obstacle-free space (a). We define the human's preference for each robot's location as the distribution over transitions in between the current and neighboring polytopes, i.e. edges on the graph. Each time the robot transitions in between sets, the set of neighbors and distribution over preferences are updated.}
\label{fig:hyperplane_arrangement}
\end{figure*}

% -------------------------------------------

\subsection{Human observation model with path preference}



%The previous human observation model is defined conditioned on the goal of the task, but not on \emph{how} to execute the task. In this work, 
% 1. Human policy: $\pi(S_{t})$ designates the human's preferred path from state $S_t$. We call human \emph{intent} at state $S_t$ the joint $\lbrace \pi(S_t),g \rbrace$.

% 2. $o_{t} = f(\pi(S_{t}), g) + \epsilon$ designates a next location $l_t$

% A possible assumption is that the user’s input noisily optimizes
% a goal-dependent cost function CG (one that depends,
% as an example, on the dot product between the user’s
% velocity and the direction to the goal). Using the principle
% of maximum entropy, we can use CG to induce a probability distribution over trajectories ξ ∈  given a goal as
% P( ξ |G) ∝ exp
% −CG( ξ )

% , in other words the probability of
% a trajectory decreases exponentially as its cost increases
% (Ziebart et al., 2008). 

% And we propose the human model
We assume that having chosen a goal and path preference, the human takes actions to noisily minimize a cost function $C_{\goal,\preference}$. For example, $C_{\goal,\preference}(\location_t, \projectedlocation_t)$ can be the length of the shortest path from location $\location_t$ to the goal $\goal$ after taking a first step to $\projectedlocation_t$, and constrained by path preference $\preference$.
% We denote $\delta ( \location_t, \goal \mid \preference)$ the optimal cost $C^{\star}_{\goal,\preference}(\location_t)$
We use $C_{\goal,\preference}$ to induce the following probability distribution over observations
% Version with delta for shortest path -----------
% \begin{equation}
%     \label{eq:humanmodel}
%     P(l_{t} \mid S_t, g, \theta)  \; \propto \; e^{-\gamma \big( (\delta(S_t \rightarrow g \mid l_t, \theta) - (\delta(S_t \rightarrow g \mid \theta) \big)}
% \end{equation}
% Version with cost (more general) -----------
\begin{equation}
    \label{eq:humanmodel}
    P(l_{t} \mid S_t, g, \theta)  \; \propto \; e^{-\gamma \big( C_{\goal,\preference}(\location_t, \projectedlocation_t) - C^{\star}_{\goal,\preference}(\location_t) \big)}.
\end{equation}
% where $\delta(a,b \mid \theta)$ designates the shortest path from locations $a$ to $b$ conditioned on preference $\theta$.
 In summary, the human will pick the lowest cost action (perhaps the shortest path) with the highest probability and the likelihood an action decreases exponentially with the increase in cost \cite{ziebart2008maximum}.

% Note that the path preference $\pi$ does not have to be a sequence of locations - it can designate a homotopy, a sequence of areas to visit...




\subsection{Inference}

At each time step where the human provides an observation, the posterior $P(g,\theta)$ is given through the bayesian update
\begin{equation}
\label{eq:inference}
    P(g,\theta \mid l_{1:t}, S_{1:t})  \; \propto \; P(l_{t} \mid S_t, g, \theta) \times P(g,\theta \mid l_{1:t-1}, S_{1:t-1}).
\end{equation}

% \begin{equation}
% \label{eq:inference}
%     P(g \mid l_{1:t}, S_{1:t})  \; \propto \; P(l_{t} \mid S_t, g) \times P(g \mid l_{1:t-1}, S_{1:t-1}).
% \end{equation}

We note that the number of bayesian updates required at each iteration to update the belief is equal to the cardinality of the joint $(\goal,\preference)$. In addition, each bayesian update involves computing $C_{\goal, \preference}(. , .)$ in Eq. \ref{eq:humanmodel}, which involves solving an optimization problem (such as a shortest path problem).
%If policy $\theta$ represents a discrete distribution over all possible paths to the goal starting from any current state, the above update is intractable. 
In Section \ref{sec:path_preference}, we propose a specific encoding of preference $\preference$ for resolving Eq. \ref{eq:inference}, while ensuring the cardinality of $(\goal,\preference)$ does not grow exponentially with the number of obstacles.




\subsection{Decision Making}

We consider a navigation problem where the robot receives reward according to the model $\mathcal{R}(\location_t, \goal, \preference, \action_t)$.
Let $b_{\goal, \preference}$ be the robot's belief distribution over the goal and preference computed from Eq. \ref{eq:inference}.
We wish to find the optimal policy $\pi$ that maximizes the expected discounted sum of future rewards.

% In practice, the robot does not know when to expect observations from the human. 
% \blue{We compute a solution supposing no observations will ever be received, and re-solve in a receding horizon as we obtain observations and update the belief.}

% \blue{Problem: The POMDP that we solve does not assume the diagram in Figure 1, as we suppose . Need to be clear on what is used for inference (figure 1), and what is used for pomdp solving.}



% Reasoning over all policies $\pi(s)$ is generally intractable. In the next section, we propose an encoding for $\pi$ for object transport problems so as to make it tractable.





% \input{tickx_graphics/BII_diagram_goal_full.tex}

% \input{tickx_graphics/BII_diagram_policy_full.tex}


% \subsection{Intention Inference with Path Preference}

% Bayesian update over b(g,pi)

% Intractable!



==> _previous_versions/2023_02_24/4_Path_Preference.tex <==



In this section, we propose an encoding of human's path preference $\preference$ for computing the posterior in Eq. \ref{eq:inference}. Differing(?) from the concept of homotopy classes, we define the preference according to a partitioning of the environment into polytopes, as shown in Figure \ref{fig:hyperplane_arrangement}, creating a \emph{hyperplane arrangement} of the space. Hyperplane arrangements have been used by \citet{vincent2021reachable} in the context of Neural Network verification.
In our setting, we leverage this representation to define path preferences as preferred transitions in between adjacent regions of the space.

% we leverage a hyperplane arrangement of the environment
% policies as being a distribution over transitions in between polyhedral regions of the obstacle-free space (shown in Figure \ref{fig:hyperplane_arrangement}). 

\subsection{Hyperplane arrangement}

We assume a two-dimensional environment composed of polytopic obstacles, each defined by their half-space representation (H-representation)
$$\mathcal{O_i} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } A_ix \leq b_i \rbrace,$$ 
where $A \in \mathbb{R}^{d_i \times 2}$ and $b \in \mathbb{R}^{d_i}$, and where $d_i$ is the number of edges (hyperplanes) composing polytope $i$. Let $n = \sum_i d_i$ be the number of hyperplanes composing the full space. 

We leverage each obstacle's H-representation to construct a hyperplane arrangement of the environment as shown in Fig. \ref{fig:hyperplane_arrangement}, i.e. a partitioning of the space into polytopes. More specifically, each location in space belongs to a polytope $j$ for which we can write an H-representation of the form
$$\mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } \forall i, \, \sign(A_ix - b_i) = \alpha^{j}_{i} \rbrace,$$
where $\alpha^{j}_{i} \in \lbrace -1,1 \rbrace^{d_i}$ is a vector specific to polytope $j$ and obstacle $i$ corresponding to the relative position of any point in the set with respect to each hyperplane in $\mathcal{O}_i$

%Each polytope can be uniquely represented by a vector $\alpha^j$.% of dimension $n$, taking on values $-1$ or $1$ according to their positions with respect to each hyperplane.
Concatenating elements from each obstacle's H-representation, we can write polytope $j$'s H-representation as 
% \begin{equation}
% \label{eq:polytope_h_representation}
% \mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } A^jx - b^j \leq 0 \rbrace,
% \end{equation}
\begin{equation}
\label{eq:polytope_h_representation}
\mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } \sign ( Ax - b ) = \alpha^j \rbrace,
\end{equation}
Where $A \in \mathbb{R}^{n \times 2}$ and $b \in \mathbb{R}^n$ are a concatenation of $A_i$ and $b_i$.%, and where the rows $a^j_k$ and $b^j_k$ correspond to 

Some of the constraints in Eq. \ref{eq:polytope_h_representation} are \emph{redundant}, i.e. the polytope does not change upon their removal. We can further reduce the H-representation of a polytope to include only non-redundant constraints:
% \begin{equation}
% \label{eq:polytope_h_representation_essential}
% \mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } A_e^jx - b_e^j \leq 0 \rbrace.
% \end{equation}
\begin{equation}
\label{eq:polytope_h_representation_essential}
\mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } \sign ( A_e^jx - b_e^j ) = \alpha_e^j \rbrace.
\end{equation}
The non-redundant constraints correspond to edges of the polytope. In other words, as the robot continually moves in space, the first hyperplane that it will cross upon exiting the polytope will correspond to one of the polytope's non-redundant constraints.
We can now characterize each polytope by a vector $\alpha^j_e \in \lbrace -1,1 \rbrace^{n_e^j}$, where $n_e^j \leq n$ is the number of essential constraints of the polytope. The polytopes $\mathcal{P}_j$ partition the environment into a \emph{hyperplane arrangement}.

\citet{vincent2021reachable} outline an iterative method for removing redundant constraints by solving $n$ linear programs. We use this method in practice for computing $\alpha_e^j$ for each polytope.







% . Let $n = \sum_i d_i$ be the number of hyperplanes composing the space. then,  

% each point in the space belongs to the intersection of half-spaces $\lbrace x \mid a^Tx \leq b \rbrace$.

% Our solution is based on an environment representation where obstacles are modeled as polyhedra. Each polyhedron has a half-space representation of the form %PH = {x ∈ R^d|Ax ≤ b}

\subsection{Graph Construction}
In this section, we provide a definition of preference $\preference$ according to a graphical representation of the environment based on the hyperplane arrangement.
Under this representation, a preference corresponds to a set of preferred transitions. In other words, for each polytope in the space, the human will have a preference on \emph{which} neighboring polytope they wish to transition to.


Remainder of this section:
\begin{enumerate}
    \item define the graph $\mathcal{G}$ derived from the hyperplane arrangement.
    \item define the mapping from a path to a sequence of edges on the graph.
    \item Property: any two paths that belong to different homotopy classes will cross different sequences of polytopes, i.e. correspond to a different sequence of edges on $\mathcal{G}$. (proof by contradiction - if they belong to the same sequence, because there are no obstacles located within each set, we can deform each path into the other portion through a continuous transformation in the set of regions that they cross -- same homotopy class)
\end{enumerate}

% (note: any hyperplane arrangement verifying the homotopy property is suitable for this application. The obstacle-defined graph has many downsides (variability of region size, dependency on irrelevent obstacle shape particularities), but the method to obtain it is computationally tractable and it applies to n-dimensional spaces. Future work would include coming up with wiser ways to compute hyperplane arrangements in a way that is relevant to the human preference and that depends less on the particular shape of obstacles.)

\subsection{Path preference}

We define a human's path preference policy as a distribution over the polytopes neighboring the current robot's location. More specifically, a human preferring neighbor $i$ will prefer paths that transition directly from the current polytope to polytope $i$.
At each iteration, only the current polytope and the neighboring polytopes condition the human's observation model. We assume the new Markov Decision Model in Figure \ref{fig:BII_diagram_decomposed_homotopies}.

Thus, at each iteration, we only need to update the components of $\pi$ that correspond to the current robot's location. For $n_g$ goals and $n_n$ neighbors, the number of measurement likelihoods to compute (and thus shortest path problems to solve) is reduced to $n_g \times n_n$.

% \subsection{Shortest path with sequence constraints}

% Assuming a goal $g$ and a preferred transition $\pi(S_t)$, computing the measurement likelihood for an observation $o_t$ requires computing the length of the shortest path from Eq \ref{eq:humanmodel}:
% \begin{equation}
%     \begin{aligned}
%     &\delta(S_t \rightarrow g \mid l_t, \pi(S_t)) \text{, and } \\
% &\delta(S_t \rightarrow g \mid \pi(S_t)).
%     \end{aligned}
% \end{equation}
% The paths must bring the robot from its current location $s_t$ to the goal $g$, constrained by sequence transition $\pi(s_t)$, and eventually passing by $l_t = f(o_t)$.

% Can be any method - $A^\star$ or $FMT^\star$ with constraints, or Tobia Marcucci's method for planning on graphs of convex sets.

% For our experiments we use $A^\star$ while pruning the invalid state transitions.


\input{tickx_graphics/BII_diagram_polytopes.tex}


==> _previous_versions/2023_02_27_1/1_Introduction.tex <==

When humans and robots collaborate and interact with each other, we expect robots to be able to quickly adapt to human decisions. Consider a ground robot navigating inside a busy room to deliver a box. It picks a path to its destination (perhaps the shortest) passing in between occupied desks. The people working at these desks may not appreciate the robot passing and interrupting their discussion. They may also want the robot to make a detour on the right so that their co-worker notices the box being delivered.
% TODO find a better wording for pb requirements (part of the objective)
These problem requirements coming from human insight and preferences have the particularity that they cannot be inferred by the robot unless people take specific actions, such as applying a force on the robot or giving a joystick instruction, to indicate the information.

We look at the problem where the robot, an imperfect, partial observer of the environment, makes navigation decisions that a human seeks to influence through recommendations. The more quickly the robot can infer the human's preference from their actions and adapt, the less effort is required from the human to do so. %(Saving the operator's time is critical...)
Solutions to this problem have been explored in the area of shared autonomy, where the robot can either \emph{infer} the human's intention given inputs, \cite{bajcsy2017learning, javdani2015shared}, correct its trajectory online \cite{hagenow2021corrective}, or leave control of a latent action space to a human operator \cite{losey2020controlling, jeon2020shared}. 


\citet{bajcsy2017learning} consider an online adaptation problem in the context of a manipulation task where a person can apply forces on the robot to indicate their preferences. For example, if the robot carries a cup of coffee too far above the ground, they will press the arm downwards and expect the robot to keep the cup at a low height even as they release it, preserving their preference while executing the task. \citet{bajcsy2017learning} frame the problem as a Partially Observable Markov Decision Process (POMDP) where parameters of the reward function are unknown a-priori and can be inferred online from human actions. %The robot's reward is a linear combination of features (e.g. tilt of the cup, or its distance to a human) with their unknown, continuous-valued weights (parameters).
We adopt a similar approach for adaptation to a human's preference in the context where a robot must autonomously navigate in a known environment, such as a cluttered office space. We focus on the particular problem where the human seeks to change the robot's \emph{path} with respect to obstacles, (e.g. contour the desks on the right). 

A common way to represent different categories of paths is using the concept of homotopy classes \cite{bhattacharya2012topological}.
However, using homotopies to encode and infer human preferences can pose computational challenges.
If the robot maintains a belief over homotopy classes for paths in between its current location and the goal, the complexity of the inference problem can grow exponentially with the number of obstacles in the space, making the resulting decision-making problem intractable. Furthermore, when the goal is also a problem unknown (which appears in prediction and shared autonomy problems such as \cite{best2015bayesian, javdani2015shared}), the number of unknown variables increases linearly with the number of candidate destinations.

% \citet{best2015bayesian} propose an interesting approach for predicting an agent's intended trajectory from observations. Rather than maintaining a belief over the agent's future path, they infer the agent's intended \emph{goal} among a set of candidate locations at the boundary of the space. This encoding of the agent's destination provides information on where it is heading, and this intention distribution is then used to generate a distribution of candidate future trajectories for the agent.

% Inferring the goal of the task among a discrete set of candidates is also relevant to the area of shared autonomy. In shared autonomy, both a person and a robot are active decision-makers and must collaborate to execute a common task. \citet{javdani2015shared} propose a problem formalism for shared control of a robotic arm, where the robot must assist the human in picking up an object but needs to infer \emph{which} object the human has chosen from joystick inputs. As the user guides the arm towards its intended object, the robot updates its belief over the candidate objects until it is confident enough to actively assist the human in picking it up.

% We argue that inferring the goal of the task and inferring a human's preferred homotopic path to a goal should be considered as separate problems. Consider the above shared autonomy scenario where the user wishes to use the robotic arm to pick up an object on the left, but prefers to get around an obstacle on the right. While providing inputs to move around the obstacle, the robot updates its belief and infers that the intended object is most likely on the right. We now face the problem where the robot is \emph{over-confident} in the wrong goal, and the robotic assistance will be more likely to pick up the wrong object. The inherent issue with this model when obstacles are present is that conditioned on a certain goal, the human's behavior is modeled as noisily rational, i.e. the human will pick the lowest cost action (perhaps the shortest path) with the highest probability and the likelihood of its action decreases exponentially with the increase in cost. In our work, we consider instead that left and right side of the obstacle are different modes among(?) which the human can have a preference. (rephrase) The robot infers the path preference jointly with the goal of the task, and we assume the human's behavior is noisily rational conditioned on both the \emph{goal} and the \emph{preference}.

This paper addresses how to encode and model a human's path preference such that a robot can update its belief over the path and goal jointly and replan online. The key to our solution is to leverage the fact that the human's actions do not contain information about the entire path at once. For example, we would push the robot on its right to indicate a preference for going around the desk in front of the robot, but this will not contain much information about how to navigate around the tables further ahead. Based on this insight, we encode a preference policy as a set of preferred transitions in between polytopes partitioning the environment and introduce conditional independence assumptions into our model that make the Bayesian inference problem tractable.% (the complexity does not increase exponentially with the number of obstacles).

Our contribution are as follows.
\begin{itemize}
    \item We formulate the human-robot collaboration problem as a Partially Observable Markov Decision Process (POMDP) where both the goal of the task and the human's path preference are unknown random variables.
    \item We propose an encoding of a human's path preference, along with conditional independence assumptions over the problem variables for inferring task goal and path preference online.
    \item (simulation results here) %(without path inference, the robot is over-confident in incorrect goal, resulting in a lower success rate compared to our solution...)
\end{itemize}




==> _previous_versions/2023_02_28/1_Introduction.tex <==

When humans and robots collaborate and interact with each other, we expect robots to be able to quickly adapt to human decisions. Consider a ground robot navigating inside a busy room to deliver a box. It picks a path to its destination (perhaps the shortest) passing in between occupied desks. The people working at these desks may not appreciate the robot passing and interrupting their discussion. They may also want the robot to make a detour on the right so that their co-worker notices the box being delivered.
These preferences coming from human insight have the particularity that they cannot be inferred by the robot unless people take specific actions, such as applying a force on the robot or giving a joystick instruction, to indicate the information.
% The point of this sentence above is to say that accounting for these preferences cannot just be done by hand-tuning the robot's objective until we find a one-size-fits-all path planner. The preferences come online from human insight that the robot does not have (the people at their desks don't want to be disturbed, but the co-worker wants to see the robot), and the robot should account for them it even though it does not know the cause.

% The robot does not know the prefer by the robot unless people take specific actions, such as applying a force on the robot or giving a joystick instruction, to indicate the information. The robot must \emph{infer} the preferences as it receives observations while executing its task.
% These preferences that the robot should account for in its problem objective
% have the particularity that they cannot be inferred by the robot unless people take specific actions, such as applying a force on the robot or giving a joystick instruction, to indicate the information.

We look at the problem where the robot, an imperfect, partial observer of the environment, makes navigation decisions that a human seeks to influence through recommendations. The more quickly the robot can infer the human's preference from their actions and adapt, the less effort is required from the human to do so. %(Saving the operator's time is critical...)


% \blue{New paragraph in construction}
Prior work has explored the problem of how to \emph{adapt} to a human's preference through indications. 
% Shared control (human operates all the time)
One category of approaches consists in sharing the control in between the robot and the human. \citet{losey2020controlling, jeon2020shared} propose a framework where control of a task-relevant latent action space is given to a human operator, and the rest is handled by an autonomous system. \citet{dragan2013policy} propose a formalism for arbitrating in between a user's input and a robot's policy when both human and robot share control of the same action space. These methods rely on a human constantly providing inputs for the robot to use. \cite{hagenow2021corrective} \blue{description to complete - corrective shared autonomy}
% Inference for the agent to be able to act on its own while accounting for the human's intention
Another category of approaches involves modeling preference as an unknown parameter of the robot's optimization problem, and inferring its value as the robot receives observations so that it can compute new solutions online \cite{javdani2015shared, bajcsy2017learning,asmar2022collaborative}. 
\citet{bajcsy2017learning} consider an online adaptation problem in the context of a manipulation task where a person can apply forces on the robot to indicate their preferences. For example, if the robot carries a cup of coffee too far above the ground, they will press the arm downwards and expect the robot to keep the cup at a low height even as they release it, preserving their preference while executing the task. By enabling the robot to continue executing its task while accounting for a probabilistic representation of human preference, we do not rely as much on receiving frequent inputs.
We adopt a similar approach for adapting to a human's preference in the context where a robot must autonomously navigate in a known environment, such as a cluttered office space. We focus on the particular problem where the human seeks to change the robot's \emph{path} with respect to obstacles, (e.g. contour the desks on the right). 

% The (inference?) problem is generally approached in three steps (rephrase). 
% First, the preference has to be \emph{encoded} into the optimization problem in a way that is relevant to the task. For example, \citet{bajcsy2017learning} model preferences as continuous-valued weights attributed to features. These features can be the distance between the robotic arm and a human operator, or the height and orientation of its end-effector.
% Second, the value of the preference must be \emph{inferred} from human inputs, which can involve computing a full belief distribution through a Bayesian update \cite{javdani2015shared} or a maximum-a-posteriori estimate of its value \cite{bajcsy2017learning}.
% Finally, the robot must re-compute solutions accounting for the updated preference parameters.

% Solutions to this problem have been explored in the area of shared autonomy, where the robot can either \emph{infer} the human's intention given inputs, \cite{bajcsy2017learning, javdani2015shared}, correct its trajectory online \cite{hagenow2021corrective}



% Solutions to this problem have been explored in the area of shared autonomy, where the robot can either \emph{infer} the human's intention given inputs, \cite{bajcsy2017learning, javdani2015shared}, correct its trajectory online \cite{hagenow2021corrective}, or leave control of a latent action space to a human operator \cite{losey2020controlling, jeon2020shared}. 


% \citet{bajcsy2017learning} consider an online adaptation problem in the context of a manipulation task where a person can apply forces on the robot to indicate their preferences. For example, if the robot carries a cup of coffee too far above the ground, they will press the arm downwards and expect the robot to keep the cup at a low height even as they release it, preserving their preference while executing the task. \citet{bajcsy2017learning} frame the problem as a Partially Observable Markov Decision Process (POMDP) where parameters of the reward function are unknown a-priori and can be inferred online from human actions. %The robot's reward is a linear combination of features (e.g. tilt of the cup, or its distance to a human) with their unknown, continuous-valued weights (parameters).
% We adopt a similar approach for adaptation to a human's preference in the context where a robot must autonomously navigate in a known environment, such as a cluttered office space. We focus on the particular problem where the human seeks to change the robot's \emph{path} with respect to obstacles, (e.g. contour the desks on the right). 

% \textbf{Encoding path preference}
A common way to represent different categories of paths is using the concept of homotopy classes \cite{bhattacharya2012topological}.
However, using homotopies to encode and infer human preferences can pose computational challenges.
If the robot maintains a belief over homotopy classes for paths in between its current location and the goal, the complexity of the inference problem can grow exponentially with the number of obstacles in the space, making the resulting decision-making problem intractable. %Furthermore, when the goal is also a problem unknown (which appears in prediction and shared autonomy problems such as \cite{best2015bayesian, javdani2015shared}), the number of unknown variables increases linearly with the number of candidate destinations.

Our solution is to encode path preference based on a partitioning of the environment into polytopes \cite{vincent2021reachable}. Over this representation, a path preference is a set of preferred transitions in between adjacent polytopes. Paths belonging to different homotopy classes correspond to different sequences of transitions.
This representation enables us to introduce conditional independence assumptions into our model that make the Bayesian inference problem tractable. The key to these assumptions is that they leverage the fact that the human's actions do not contain information about the entire path at once. For example, we would push the robot on its right to indicate a preference for going around the desk in front of the robot, but this will not contain much information about how to navigate around the tables further ahead. 
Finally, after updating its belief representation over the human's preference, the robot can adapt to indications by replanning online.
% Our solution has the particularity that paths belonging to different homotopy classes correspond to different preferences.
%By introducing these assumptions, we prevent the complexity of the Bayesian Update step from increasing with the number of obstacles in the environment.
% \blue{need to finish: how we make the inference problem scalable through conditional independence assumptions...}


% This paper addresses how to encode and model a human's path preference such that a robot can update its belief over the path and goal jointly and replan online. The key to our solution is to leverage the fact that the human's actions do not contain information about the entire path at once. For example, we would push the robot on its right to indicate a preference for going around the desk in front of the robot, but this will not contain much information about how to navigate around the tables further ahead. Based on this insight, we encode a preference policy as a set of preferred transitions in between polytopes partitioning the environment and introduce conditional independence assumptions into our model that make the Bayesian inference problem tractable.% (the complexity does not increase exponentially with the number of obstacles).

Our contribution are as follows.
\begin{itemize}
    \item We formulate the human-robot collaboration problem as a Partially Observable Markov Decision Process (POMDP) where both the goal of the task and the human's path preference are unknown random variables.
    \item We propose an encoding of a human's path preference, along with conditional independence assumptions over the problem variables for inferring task goal and path preference online.
    \item (simulation results here) %(without path inference, the robot is over-confident in incorrect goal, resulting in a lower success rate compared to our solution...)
\end{itemize}




==> _previous_versions/2023_02_28/2_Related_Work.tex <==

\citet{best2015bayesian} propose an interesting approach for predicting an agent's intended trajectory from observations. Rather than maintaining a belief over the agent's future path, they infer the agent's intended \emph{goal} among a set of candidate locations at the boundary of the space. This encoding of the agent's destination provides information on where it is heading, and this intention distribution is then used to generate a distribution of candidate future trajectories for the agent.

Inferring the goal of the task among a discrete set of candidates is also relevant to the area of shared autonomy. In shared autonomy, both a person and a robot are active decision-makers and must collaborate to execute a common task. \citet{javdani2015shared} propose a problem formalism for shared control of a robotic arm, where the robot must assist the human in picking up an object but needs to infer \emph{which} object the human has chosen from joystick inputs. As the user guides the arm towards its intended object, the robot updates its belief over the candidate objects until it is confident enough to actively assist the human in picking it up.

We argue that inferring the goal of the task and inferring a human's preferred path to a goal should be considered as separate problems. Consider the above shared autonomy scenario where the user wishes to use the robotic arm to pick up an object on the left, but prefers to get around an obstacle on the right. While providing inputs to move around the obstacle, the robot updates its belief and infers that the intended object is most likely on the right. We now face the problem where the robot is \emph{over-confident} in the wrong goal, and the robotic assistance will be more likely to pick up the wrong object.
In an environment containing obstacles, assuming that the human's behavior is noisily rational conditioned only on the goal will lead to similar over-confident behaviors.
%By noisily rational, the human will pick the lowest cost action (perhaps the shortest path) with the highest probability and the likelihood an action decreases exponentially with the increase in cost. 
In our work, we consider instead that left and right side of the obstacle are modes corresponding to different homotopy classes, one of which is preferred by the human. The robot infers the path preference jointly with the goal of the task, and we assume the human's behavior is noisily rational conditioned on both the goal and the preference.


Two trajectories belong to the same homotopy class if one can be deformed smoothly into the other without intersecting an obstacle \cite{bhattacharya2012topological}. Planning with homotopy class constraints is useful in problems where the robot's requirements are given with respect to obstacles. For example, \cite{yi2016homotopy} consider topological constraints provided by human operators of the form “go quickly from A to B while avoiding C”. \citet{Bhattacharya_2010} propose an efficient algorithm for solving path planning problems under homotopic constraints that can apply to such scenarios.
Unfortunately, the number of homotopy classes for a given problem can be infinite, which makes it challenging to carry out inference over homotopy classes directly. In addition, homotopies are defined for a given set of obstacles and for a specific start and goal locations. As the robot changes location and updates its representation of the world, carrying out inference over homotopy classes in a dynamic environment requires re-computing the set of homotopies at every iteration, making the belief update challenging.
% Our solution is to propose an encoding for path preference based on a partitioning of the obstacle-free space into polytopes \cite{vincent2021reachable}, with the particularity that paths belonging to different homotopy classes correspond to different preferences.


% homotopies from start to goal. Downsides:
% - shortest path homotopies are not always the most relevant
% - homotopy is defined with respect to a start and a goal, and these need to be re-defined as the robot moves, which is especially challenging. In addition, as the number of candidate goals increases, the number of homotopies increase linearly as well (one set of them per goal)
% - Each obstacle adds a new dimension to the problem (for astar with homotopy work), making the complexity increase exponentially with the number of obstacles.


==> _previous_versions/2023_02_28/3_Problem_Statement.tex <==

% NOTATIONS
\newcommand{\location}{S} %
\newcommand{\goal}{g} %
\newcommand{\goalset}{\mathcal{C}_{\goal}}
\newcommand{\preference}{\theta}
\newcommand{\preferenceset}{\Theta}
\newcommand{\action}{a}
\newcommand{\actionspace}{\mathcal{A}}
\newcommand{\observation}{o}
\newcommand{\projectedlocation}{S^{(i)}}



\input{tickx_graphics/BII_diagram_policy_full.tex}

We consider a robot that is tasked to navigate in a known environment to an unknown destination. A human knows the destination and can intervene with a joystick or apply force cues to provide a heading direction to the robot \textcolor{purple}{Mac: Or provide force cues?  Let's be consistent throughout.}. The human also has a preference on which \emph{path}, with respect to obstacles, the robot should take to get to the goal. Our objective is for the robot to understand the human's intentions and execute the intended task while requiring a minimal amount of interventions.



% -------------------------------------------
%Figure placement
\begin{figure*}
\subfloat[width=6cm][Hyperplane arrangement of a two-dimensional space containing two obstacles (colored in gray). The robot is located inside the pink polytope, surrounded by three adjacent obstacle-free polytopes. Each hyperplane on the boundary of the robot's polytope corresponds to one of the non-redundant constraints in Eq. \ref{eq:polytope_h_representation_essential}.]{\resizebox{0.65\columnwidth}{!}{%
\includegraphics[]{figures/hyperplane_arrangement.PNG}}\label{fig:HA}} 
\quad
\subfloat[width=6cm][Graph derived from hyperplane arrangement. The nodes on the graph designate polytopes, and edges designate transitions to adjacent polytopes. To estimate the human's preference, the robot updates a posterior over the goal polytope and one-step transitions $p_1$, $p_2$ and $p_3$ given all human inputs up to that time.]{\resizebox{0.65\columnwidth}{!}{%
\includegraphics[]{figures/HA_graph.PNG}}\label{fig:HA_graph}}
\quad
\subfloat[width=6cm][Example preference defined over the graph. The location of the goal is indicated with the yellow pentagon in the lower right polytope. For each node, the outgoing pink arrow designates the edge on the graph corresponding to the preferred transition between polytopes.]{\resizebox{0.65\columnwidth}{!}{%
\includegraphics[]{figures/HA_pref.PNG}}\label{fig:HA_pref}}
\caption{Using the hyperplanes composing the H-representation of each obstacle, we construct a hyperplane arrangement of the obstacle-free space (a). We define the human's preference for the robot's one step action choices as the posterior distribution (given all human input up to that point) over transitions from the current to the neighboring polytopes, i.e. edges on the graph. Each time the robot transitions to a new polytope, the set of neighbor polytopes and the distribution over human preferences are updated.}
\label{fig:hyperplane_arrangement}
\end{figure*}

% -------------------------------------------


Let $\goal$ be a random variable designating the goal of the task. $\goal$ belongs to a discrete set of candidates $\goalset$.
Let $\preference$ be the human's path preference, represented as a discrete-valued random variable. \textcolor{purple}{Mac: represented as what?}. We denote $\preferenceset$ the set of possible preferences.
Let $\location_t \in \mathbb{R}^2$ be the physical location of the robot and $\action_t$ the robot's action, belonging to some action space $\actionspace$ at time index $t$ \textcolor{blue}{Mac: How are state and action represented?  Continuous or discrete?}. The transition model $T(\location_{t+1} \mid \location_t,\action_t)$ is deterministic: the robot has full control over its future location. At any time step, the human may provide observations for the robot. When a human intervenes (either with a joystick or by applying forces on the robot), the robot receives an observation $\observation_t$ corresponding to a direction (i.e. heading angle). Taking one step in direction $\observation_t$ from location $\location_t$  %\textcolor{purple}{Mac: notation, why is the new state $l_t$?  Why not $S_{t+1}$ or something else the uses $S$?} 
brings the robot 
%\textcolor{purple}{Mac: First mention of an object?  Let's just say the robot.  We can say in the intro that it may be carrying an object.}%Object was a remnant of an old version of the paper and shouldn't appear
to a new location $\projectedlocation_t$ in space.

% \subsection{Human observation model with path preference}

We assume the robot has available a stochastic observation model for the human $\mathcal{O}(\observation_t \mid \location_t, \goal, \preference)$ conditioned both on the goal of the task $\goal$, and the human's preferred path $\preference$.  
%\textcolor{purple}{Mac: Where does this model come from?  If we suppose a specific form, can we give the form here, and justify it?} 
More specifically, we assume that having chosen a goal and path preference, the human takes actions to noisily minimize a cost function $C_{\goal,\preference}$. For example, $C_{\goal,\preference}(\location_t, \projectedlocation_t)$ can be the length of the shortest path from location $\location_t$ to the goal $\goal$ after taking a first step to $\projectedlocation_t$, and constrained by path preference $\preference$.
% We denote $\delta ( \location_t, \goal \mid \preference)$ the optimal cost $C^{\star}_{\goal,\preference}(\location_t)$
We use $C_{\goal,\preference}$ to induce the following probability distribution over observations
% Version with delta for shortest path -----------
% \begin{equation}
%     \label{eq:humanmodel}
%     P(l_{t} \mid S_t, g, \theta)  \; \propto \; e^{-\gamma \big( (\delta(S_t \rightarrow g \mid l_t, \theta) - (\delta(S_t \rightarrow g \mid \theta) \big)}
% \end{equation}
% Version with cost (more general) -----------
\begin{equation}
    \label{eq:humanmodel}
    P(l_{t} \mid S_t, g, \theta)  \; \propto \; e^{-\gamma \big( C_{\goal,\preference}(\location_t, \projectedlocation_t) - C^{\star}_{\goal,\preference}(\location_t) \big)}.
\end{equation}
% where $\delta(a,b \mid \theta)$ designates the shortest path from locations $a$ to $b$ conditioned on preference $\theta$.
 In summary, the human will pick the lowest cost action (perhaps the shortest path) with the highest probability and the likelihood of an action decreases exponentially with the increase in cost \cite{ziebart2008maximum}. Our inclusion of the the path preference $\preference$ set our approach apart from, for example, \cite{best2015bayesian}. The model is shown in Figure \ref{fig:BII_diagram_policy_obs} represented as a Bayesian Network.




\subsection{Inference}

At each time step where the human provides an observation, the posterior $P(g,\theta)$ is given through the bayesian update
\begin{equation}
\label{eq:inference}
    P(g,\theta \mid l_{1:t}, S_{1:t})  \; \propto \; P(l_{t} \mid S_t, g, \theta) \times P(g,\theta \mid l_{1:t-1}, S_{1:t-1}).
\end{equation}
% \begin{equation}
% \label{eq:inference}
%     P(g \mid l_{1:t}, S_{1:t})  \; \propto \; P(l_{t} \mid S_t, g) \times P(g \mid l_{1:t-1}, S_{1:t-1}).
% \end{equation}
We note that the number of bayesian updates required at each iteration to update the belief is equal to the cardinality of the joint $(\goalset,\preferenceset)$. In addition, each bayesian update involves computing $C_{\goal, \preference}(. , .)$ in Eq. \ref{eq:humanmodel}, which involves solving an optimization problem (such as a shortest path problem).
%If policy $\theta$ represents a discrete distribution over all possible paths to the goal starting from any current state, the above update is intractable. 
In Section \ref{sec:path_preference}, we propose a specific encoding of preference $\preference$ for resolving Eq. \ref{eq:inference}, while ensuring the number of computations of the cost $C_{\goal, \preference}(. , .)$ per update does not grow exponentially with the number of obstacles.




\subsection{Decision Making}

We consider a navigation problem where the robot receives reward according to the model $\mathcal{R}(\location_t, \goal, \preference, \action_t)$.
%Let $b_{\goal, \preference}$ be the robot's belief distribution over the goal and preference computed from Eq. \ref{eq:inference}.
Let $\mathcal{S}=(\mathbb{R}^2,\goalset,\preferenceset)$ be the set of possible states composed of the robot's location, the problem goal and the human's preference. 
We wish to find the optimal policy $\pi$ that maximizes the expected discounted sum of future rewards. We writs $\gamma$ the discount factor for the reward.
The above problem is a Partially Observable Markov Decision Process described by the tuple $(\mathcal{S}, \actionspace, \mathcal{O}, T, \mathcal{R}, \gamma)$ \cite{kochenderfer2015decision}.

% In practice, the robot does not know when to expect observations from the human. 
% \blue{We compute a solution supposing no observations will ever be received, and re-solve in a receding horizon as we obtain observations and update the belief.}

% \blue{Problem: The POMDP that we solve does not assume the diagram in Figure 1, as we suppose . Need to be clear on what is used for inference (figure 1), and what is used for pomdp solving.}





==> _previous_versions/2023_02_28/4_Path_Preferences.tex <==

In this section, we propose an encoding of human's path preference $\preference$ for computing the posterior in Eq. \ref{eq:inference}. Deviating from the concept of homotopy classes, we define the preference according to a partitioning of the environment into polytopes, as shown in Figure \ref{fig:hyperplane_arrangement}, creating a \emph{hyperplane arrangement} of the space. Hyperplane arrangements have been used by \citet{vincent2021reachable} in the context of Neural Network verification.
In our setting, we leverage this representation to define path preferences as preferred transitions in between adjacent regions of the space.


\subsection{Hyperplane arrangement}

\input{tickx_graphics/BII_diagram_polytopes.tex}

We assume a two-dimensional environment composed of polytopic obstacles, each defined by their half-space representation (H-representation)
$$\mathcal{O_i} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } A_ix \leq b_i \rbrace,$$ 
where $A \in \mathbb{R}^{d_i \times 2}$ and $b \in \mathbb{R}^{d_i}$, and where $d_i$ is the number of edges (hyperplanes) composing polytope $i$. Let $n = \sum_i d_i$ be the number of hyperplanes composing the full space. 

We leverage each obstacle's H-representation to construct a hyperplane arrangement of the environment as shown in Fig. \ref{fig:hyperplane_arrangement}, i.e. a partitioning of the space into polytopes. More specifically, each location in space belongs to a polytope $j$ for which we can write an H-representation of the form
$$\mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } \forall i, \, \sign(A_ix - b_i) = \alpha^{j}_{i} \rbrace,$$
where $\alpha^{j}_{i} \in \lbrace -1,1 \rbrace^{d_i}$ is a vector specific to polytope $j$ and obstacle $i$ corresponding to the relative position of any point in the set with respect to each hyperplane in $\mathcal{O}_i$.

%Each polytope can be uniquely represented by a vector $\alpha^j$.% of dimension $n$, taking on values $-1$ or $1$ according to their positions with respect to each hyperplane.
Concatenating elements from each obstacle's H-representation, we can write polytope $j$'s H-representation as 
% \begin{equation}
% \label{eq:polytope_h_representation}
% \mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } A^jx - b^j \leq 0 \rbrace,
% \end{equation}
\begin{equation}
\label{eq:polytope_h_representation}
\mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } \sign ( Ax - b ) = \alpha^j \rbrace,
\end{equation}
Where $A \in \mathbb{R}^{n \times 2}$ and $b \in \mathbb{R}^n$ are a concatenation of $\lbrace A_i \rbrace_{\forall i}$ and $ \lbrace b_i \rbrace_{\forall i}$ respectively.%, and where the rows $a^j_k$ and $b^j_k$ correspond to 

Some of the constraints in Eq. \ref{eq:polytope_h_representation} are \emph{redundant}, i.e. the set $\mathcal{P}_j$ does not change upon their removal. We can further reduce the H-representation of a polytope to include only non-redundant constraints:
% \begin{equation}
% \label{eq:polytope_h_representation_essential}
% \mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } A_e^jx - b_e^j \leq 0 \rbrace.
% \end{equation}
\begin{equation}
\label{eq:polytope_h_representation_essential}
\mathcal{P_j} = \lbrace x \in \mathbb{R}^2 \text{ s.t. } \sign ( A_e^jx - b_e^j ) = \alpha_e^j \rbrace.
\end{equation}
The non-redundant constraints correspond to edges of the polytope. In other words, as the robot continually moves in space, the first hyperplane that it will cross upon exiting the polytope will correspond to one of the polytope's non-redundant constraints.
We can now characterize each polytope by a vector $\alpha^j_e \in \lbrace -1,1 \rbrace^{n_e^j}$, where $n_e^j \leq n$ is the number of essential constraints of the polytope. The polytopes $\mathcal{P}_j$ partition the environment into a \emph{hyperplane arrangement}.

\citet{vincent2021reachable} outline an iterative method for removing redundant constraints by solving $n$ linear programs. We use this method in practice for computing $\alpha_e^j$ for each polytope.







% . Let $n = \sum_i d_i$ be the number of hyperplanes composing the space. then,  

% each point in the space belongs to the intersection of half-spaces $\lbrace x \mid a^Tx \leq b \rbrace$.

% Our solution is based on an environment representation where obstacles are modeled as polyhedra. Each polyhedron has a half-space representation of the form %PH = {x ∈ R^d|Ax ≤ b}

\subsection{Path Preference}
In this section, we provide a definition of preference $\preference$ according to a graphical representation of the environment based on the hyperplane arrangement.
Under this representation, a path preference corresponds to a set of preferred transitions. In other words, for each polytope in the space, the human will have a preference on \emph{which} neighboring polytope they wish to transition to.

Let $\mathcal{G}$ be an undirected graph composed of vertices $v \in \mathcal{V}$, corresponding to obstacle-free polytopes, and edges $e \in \mathcal{E}$ corresponding to transitions in between adjacent polytopes. Each polytope is described by a unique vector $\alpha_e^j$ as defined in \ref{eq:polytope_h_representation_essential}. Two polytopes are adjacent if they share non-redundant constraints corresponding to the same hyperplane (i.e. they are on opposite sides of the hyperplane).
Let $\mathcal{N}(v)$ be the set of neighbors of a vertex $v$. For each vertex, we denote $p_v$ the discrete-valued random variable describing which edge in $\mathcal{N}(v)$ the human intends to transition to.

Using this formalism, we define a path preference as the set of preferred transitions over all nodes in the graph,
\begin{equation}
    \label{eq:preference}
    \preference = \lbrace p_v, v \in \mathcal{V} \rbrace.
\end{equation}

Let $m_\preference = \sum_{v \in \mathcal{V}} \vert \mathcal{N}(v) \vert = 2 \vert \mathcal{E} \vert $ be the cardinality of $\preferenceset$, and $m_\goal = \vert \mathcal{C_g} \vert$ the number of possible goals. Then the number of Bayesian updates required to update the belief at every iteration is $m_\preference \times m_\goal$.

Now, let us assume the new problem diagram in Figure~\ref{fig:BII_diagram_decomposed_homotopies}. More specifically, we introduce the assumption that conditioned on a robot location $\location_t$, the goal $\goal$, and the preference for the corresponding vertex $p_v$ in the graph, the observation $o_t$ and the preference for any other vertex are conditionally independent. In other words, the observations the human provides can be defined conditioned only on the robot location, the goal, and the human's preference for its current vertex $p_v$. By introducing this assumption, each update step only requires updating the joint $(p_v, \goal)$, reducing the number of cost computations to $\vert \mathcal{N}(v) \vert \times m_\goal$. We can notice that by introducing this assumption, we removed the direct relationship in between the number of polytopes in the environment and the complexity of the Bayesian update in Eq. \ref{eq:inference}.


% Thus, at each iteration, we only need to update the components of $\theta$ that correspond to the current robot's location. For $n_g$ goals and $n_n$ neighbors, the number of measurement likelihoods to compute (and thus shortest path problems to solve) is reduced to $n_g \times n_n$.

% We assume the new problem diagram in Figure \ref{fig:BII_diagram_decomposed_homotopies}.

In practice, components of $\preference$ are not mutually independent. For example, if the human preference at a vertex $v_1$ is $p_{v1}~=~(v_1,v_2)$, it is unlikely that the human will also prefer $p_{v_2}~=~(v_2, v_1)$ (turning back). We can improve our model by assuming a dependence relationship in between preferences for adjacent edges, which does not significantly increase the complexity of the inference problem.

 % In Figure \ref{fig:hyperplane_arrangement} showing an example preference policy given a goal, we assumed that the preferences would \emph{lead to} the goal, even without corresponding to the shortest path.




% (note: any hyperplane arrangement verifying the homotopy property is suitable for this application. The obstacle-defined graph has many downsides (variability of region size, dependency on irrelevent obstacle shape particularities), but the method to obtain it is computationally tractable and it applies to n-dimensional spaces. Future work would include coming up with wiser ways to compute hyperplane arrangements in a way that is relevant to the human preference and that depends less on the particular shape of obstacles.)



An interesting property of our encoding is that any two paths that belong to different homotopy classes will cross different sequences of polytopes, i.e. correspond to a different sequence of edges on $\mathcal{G}$.
This can be proved by contradiction. Let us suppose that two continuous trajectories, $\xi_1$ and $\xi_2$, traverse the same regions in $\mathcal{G}$ and transition through the same edges in the same order, and do not traverse any obstacle. This implies that each region the paths traverse is obstacle-free. Therefore, within each polytope, there is no obstacle in the area located in between the portions of $\xi_1$ and $\xi_2$ that belong to the region. \blue{finish and rephrase Because the trajectories are continuous, each portion is attached to the other at the edge of each polytope%Consider the space defined by the union of polytopes traversed by 
Because trajectories $\xi_1$ and $\xi_2$ are never separated by an obstacle, they can be continually deformed into one another, and thus belong to the same homotopy class. }

% (proof by contradiction - if they belong to the same sequence, because there are no obstacles located within each set, we can deform each path into the other portion through a continuous transformation in the set of regions that they cross -- same homotopy class)

% \subsection{Shortest path with sequence constraints}

% Assuming a goal $g$ and a preferred transition $\pi(S_t)$, computing the measurement likelihood for an observation $o_t$ requires computing the length of the shortest path from Eq \ref{eq:humanmodel}:
% \begin{equation}
%     \begin{aligned}
%     &\delta(S_t \rightarrow g \mid l_t, \pi(S_t)) \text{, and } \\
% &\delta(S_t \rightarrow g \mid \pi(S_t)).
%     \end{aligned}
% \end{equation}
% The paths must bring the robot from its current location $s_t$ to the goal $g$, constrained by sequence transition $\pi(s_t)$, and eventually passing by $l_t = f(o_t)$.

% Can be any method - $A^\star$ or $FMT^\star$ with constraints, or Tobia Marcucci's method for planning on graphs of convex sets.

% For our experiments we use $A^\star$ while pruning the invalid state transitions.





==> draft.tex <==
Enjeu: 
 - Solving only for the desired human goal in shared autonomy is not enough [because...]. 
 Solution in the literature: We can blend in human input (predict and blend). However, in many human-robot cooperation settings, the human may not be capable of providing a rich enough input that the robot can blend into a safe and desirable action. [Example of table pushing].
 Thus, we propose to reason about the human desired trajectory in addition to their goal destination, and find a policy that can better suit the user and facilitate task completion.

Pillars of this problem:

Shared autonomy with an unknown destination formulated as a Markov Decision Process

Bayesian Intention Inference for Trajectory and Goal Prediction

Contributions:
 - We establish a two-level planner: high level grid+POMCP, and lower level distributed multi-robot controller. The results of the high-level planner are directly integrated into the cost function of the lower level optimal planner.
  - We use POMCP (instead of Hindsight Optimization in the literature) to take information gathering actions, which we claim is preferable in settings where human input is impoverished
 (- We distribute POMCP solving using distributed MCTS)
 - We build upon BII paper to infer both where the goal is, given the human input, where the human pushes along a desired trajectory and not immediately towards the goal

==> tickx_graphics/BII_diagram_goal_full.tex <==

\begin{figure}
\label{fig:BII_diagram_traditional_obs}
\begin{tikzpicture}[->,>=stealth',auto,node distance=2.5cm,
  thick]
  
  \tikzstyle{dots} = [circle,text centered]
  \tikzstyle{state} = [circle,draw,fill=black!5, minimum size=1.2cm]
  \tikzstyle{observation} = [circle,draw,fill=blue!5, minimum size=1.2cm]
  \tikzstyle{belief} = [circle,draw,fill=orange!5, minimum size=1.2cm]

  \node[dots] (1) {\dots};
  \node[state] (2) [right of=1] {$S_{t-1}$};
  \node[state] (3) [right of=2] {$S_t$};
  \node[state] (4) [right of=3] {$S_{t+1}$};
  \node[dots] (5) [right of=4] {\dots};
  
  \node[observation] (6) [below of=2] {$o_{t-1}$};
  \node[observation] (7) [below of=3] {$o_t$};
  \node[observation] (8) [below of=4] {$o_{t+1}$};
  
%   \node[belief] (goal) [above of=3] {$g$};
  \node[belief] (goal) [below of=7] {$g$};

  \path[every node/.style={font=\sffamily\small}]
    (1) edge node [right] {} (2)
    (2) edge node [right] {} (3)
    (3) edge node [right] {} (4)
    (4) edge node [right] {} (5)
    (2) edge node [below] {} (6)
    (3) edge node [below] {} (7)
    (4) edge node [below] {} (8)
    % (goal) edge node [left] {} (3)
    % (goal) edge node [right] {} (4)
    % (goal) edge node [left] {} (2);
    (goal) edge node [left] {} (6)
    (goal) edge node [right] {} (7)
    (goal) edge node [left] {} (8);
    %(4) edge[bend right] node [left] {} (1);
    % (goal) edge [bend right] node [left] (3)
    
    
    \draw [dotted, draw=gray, ->] (goal) -- (2);
    \draw [dotted, draw=gray, ->] (goal) to [bend right] (3);
    \draw [dotted, draw=gray, ->] (goal) -- (4);

\end{tikzpicture}
\caption{Traditional intent inference model.% for trajectory prediction. 
The goal vector captures the robot's belief of the human's intended goal. The dotted lines represent the case where the human's actions have an direct effect on the robot's motion.}
\end{figure}


% \begin{figure}
% \label{BII_diagram_traditional}
% \begin{tikzpicture}[->,>=stealth',auto,node distance=2.5cm,
%   thick]
  
%   \tikzstyle{dots} = [circle,text centered]
%   \tikzstyle{state} = [circle,draw,fill=black!5, minimum size=1.2cm]
%   \tikzstyle{belief} = [circle,draw,fill=orange!5, minimum size=1.2cm]

%   \node[dots] (1) {\dots};
%   \node[state] (2) [right of=1] {$S_{t-1}$};
%   \node[state] (3) [right of=2] {$S_t$};
%   \node[state] (4) [right of=3] {$S_{t+1}$};
%   \node[dots] (5) [right of=4] {\dots};
  
%   \node[belief] (goal) [above of=3] {$g$};

%   \path[every node/.style={font=\sffamily\small}]
%     (1) edge node [right] {} (2)
%     (2) edge node [right] {} (3)
%     (3) edge node [right] {} (4)
%     (4) edge node [right] {} (5)
%     (goal) edge node [left] {} (3)
%     (goal) edge node [right] {} (4)
%     (goal) edge node [left] {} (2);
%     %(4) edge[bend right] node [left] {} (1);
% \end{tikzpicture}
% \caption{Traditional intent inference model for trajectory prediction. The goal vector captures the robot's belief of the human's intended goal.}
% \end{figure}


==> tickx_graphics/BII_diagram_policy_combined.tex <==

\begin{figure}
\label{fig:BII_diagram_policy_combined}
\subfloat[width=5cm][Goal inference model.]{\resizebox{0.5\columnwidth}{!}{%
\begin{tikzpicture}[->,>=stealth',auto,node distance=2.5cm,
  thick]
  
  \tikzstyle{dots} = [circle,text centered]
  \tikzstyle{state} = [circle,draw,fill=black!5, minimum size=1.2cm]
  \tikzstyle{observation} = [circle,draw,fill=blue!5, minimum size=1.2cm]
  \tikzstyle{belief} = [circle,draw,fill=orange!5, minimum size=1.2cm]

  \node[dots] (1) {\dots};
  \node[state] (2) [right of=1, left=2mm] {$S_{t-1}$};
  \node[state] (3) [right of=2] {$S_t$};
  \node[state] (4) [right of=3] {$S_{t+1}$};
  \node[dots] (5) [right of=4, left=3mm] {\dots};
  
  \node[observation] (6) [below of=2] {$o_{t-1}$};
  \node[observation] (7) [below of=3] {$o_t$};
  \node[observation] (8) [below of=4] {$o_{t+1}$};
  
%   \node[belief] (goal) [above of=3] {$g$};
  \node[belief] (goal) [below of=7] {$g$};

  \path[every node/.style={font=\sffamily\small}]
    (1) edge node [right] {} (2)
    (2) edge node [right] {} (3)
    (3) edge node [right] {} (4)
    (4) edge node [right] {} (5)
    (2) edge node [below] {} (6)
    (3) edge node [below] {} (7)
    (4) edge node [below] {} (8)
    % (goal) edge node [left] {} (3)
    % (goal) edge node [right] {} (4)
    % (goal) edge node [left] {} (2);
    (goal) edge node [left] {} (6)
    (goal) edge node [right] {} (7)
    (goal) edge node [left] {} (8);
    %(4) edge[bend right] node [left] {} (1);
    % (goal) edge [bend right] node [left] (3)
    
    
    \draw [dotted, draw=gray, ->] (goal) -- (2);
    \draw [dotted, draw=gray, ->] (goal) to [bend right] (3);
    \draw [dotted, draw=gray, ->] (goal) -- (4);

\end{tikzpicture}}\label{<figure1>}} 
% \quad
\subfloat[width=5cm][Intent inference model with path preferences. ]{\resizebox{0.5\columnwidth}{!}{%
\begin{tikzpicture}[->,>=stealth',auto,node distance=2.5cm,
  thick]
  
  \tikzstyle{dots} = [circle,text centered]
  \tikzstyle{state} = [circle,draw,fill=black!5, minimum size=1.2cm]
  \tikzstyle{observation} = [circle,draw,fill=blue!5, minimum size=1.2cm]
  \tikzstyle{belief} = [circle,draw,fill=orange!5, minimum size=1.2cm]

  \node[dots] (1) {\dots};
  \node[state] (2) [right of=1, left=2mm] {$S_{t-1}$};
  \node[state] (3) [right of=2] {$S_t$};
  \node[state] (4) [right of=3] {$S_{t+1}$};
  \node[dots] (5) [right of=4, left=3mm] {\dots};
  
  \node[observation] (6) [below of=2] {$o_{t-1}$};
  \node[observation] (7) [below of=3] {$o_t$};
  \node[observation] (8) [below of=4] {$o_{t+1}$};
  
%   \node[belief] (goal) [above of=3] {$g$};
  \node[belief] (goal) [below of=7] {$g, \theta$};

  \path[every node/.style={font=\sffamily\small}]
    (1) edge node [right] {} (2)
    (2) edge node [right] {} (3)
    (3) edge node [right] {} (4)
    (4) edge node [right] {} (5)
    (2) edge node [below] {} (6)
    (3) edge node [below] {} (7)
    (4) edge node [below] {} (8)
    % (goal) edge node [left] {} (3)
    % (goal) edge node [right] {} (4)
    % (goal) edge node [left] {} (2);
    (goal) edge node [left] {} (6)
    (goal) edge node [right] {} (7)
    (goal) edge node [left] {} (8);
    %(4) edge[bend right] node [left] {} (1);
    % (goal) edge [bend right] node [left] (3)
    
    
    \draw [dotted, draw=gray, ->] (goal) -- (2);
    \draw [dotted, draw=gray, ->] (goal) to [bend right] (3);
    \draw [dotted, draw=gray, ->] (goal) -- (4);

\end{tikzpicture}}\label{fig:BII_policy_only}}
\caption{Intent inference model without (left) and with (right) path preferences. The goal vector captures the robot's belief of the human's intended goal. The dotted lines represent the direct effect of the human's actions on the robot's motion (e.g. human forces or feed-forward control term). The belief in the human's preferred policy is modeled as a discrete probability distribution over the set of all possible sequences for the solution for each robot location.}
\end{figure}


